Learning latent representations for operational nitrogen response rate prediction

Learning latent representations has aided operational decision-making in several disciplines. Its advantages include uncovering hidden interactions in data and automating procedures which were performed manually in the past. Representation learning is also being adopted by earth and environmental sciences. However, there are still subfields that depend on manual feature engineering based on expert knowledge and the use of algorithms which do not utilize the latent space. Relying on those techniques can inhibit operational decision-making since they impose data constraints and inhibit automation. In this work, we adopt a case study for nitrogen response rate prediction and examine if representation learning can be used for operational use. We compare a Multilayer Perceptron, an Autoencoder, and a dual-head Autoencoder with a reference Random Forest model for nitrogen response rate prediction. To bring the predictions closer to an operational setting we assume absence of future weather data, and we are evaluating the models using error metrics and a domain-derived error threshold. The results show that learning latent representations can provide operational nitrogen response rate predictions by offering performance equal and sometimes better than the reference model.

==> metric_table.tex <==
\begin{table}[t]
\caption{The parameters tuned during Bayesian optimization for Random Forest.}
\label{tab:metrics}
\begin{center}
\begin{tabular}{l|cccc|cccc}
\multicolumn{1}{c}{\bf }  &\multicolumn{4}{c}{\bf Waiotu} &\multicolumn{4}{c}{\bf Mahana}\\
\multicolumn{1}{c}{\bf Predictions considered}  &\multicolumn{2}{c}{\bf Random Forest} &\multicolumn{2}{c}{\bf Dual-head autoencoder} &\multicolumn{2}{c}{\bf Random Forest} &\multicolumn{2}{c}{\bf Dual-head autoencoder}\\
\multicolumn{1}{c}{\bf }  &\multicolumn{1}{c}{\bf MAE} &\multicolumn{1}{c}{\bf $R^2$} &\multicolumn{1}{c}{\bf MAE} &\multicolumn{1}{c}{\bf $R^2$} &\multicolumn{1}{c}{\bf MAE} &\multicolumn{1}{c}{\bf $R^2$} &\multicolumn{1}{c}{\bf MAE} &\multicolumn{1}{c}{\bf $R^2$}
\\ \hline \\
Non-irrigated                  & 2.02 & 0.51 & 2.05 & 0.51 & 2.75 & 0.4  & 2.76 & 0.32\\
Irrigated                      & 1.09 & 0.87 & 1.41 & 0.79 & 0.99 & 0.92 & 1.1  & 0.89\\
Non-irrigated (Summer months)  & \cellcolor{blue!25}3.25 & \cellcolor{blue!25}0.03 & \cellcolor{green!25}2.91 & \cellcolor{green!25}0.04 & \cellcolor{blue!25}5.2  & \cellcolor{blue!25}0.03 & \cellcolor{green!25}4.4  & \cellcolor{green!25}0.1\\
Irrigated (Summer months)      & 0.93 & 0.76 & 1.08 & 0.64 & 0.91 & 0.57 & 0.98 & 0.51\\
\end{tabular}
\end{center}
\end{table}

==> wilcoxon_table.tex <==
\begin{table}[t]
\caption{Wilcoxon signed rank test results. On column 'Predictions considered' we note the nitrogen response rate predictions included each time on the test by each algorithm. The asterisk denotes the cases where the difference of the distributions of the predictions is statistically significant.}
\label{tab:wilcoxon}
\begin{center}
\begin{tabular}{lcc}
\multicolumn{1}{c}{\bf Predictions considered}  &\multicolumn{1}{c}{\bf Waiotu} &\multicolumn{1}{c}{\bf Mahana} 
\\ \hline \\
    Non-irrigated                       & *   & *\\
    Irrigated                           & *   & *\\
    Non-irrigated (Summer months)       & *   & *\\
    Irrigated (Summer months)           & *   & *\\
\end{tabular}
\end{center}
\end{table}
